A Survey on Benchmarks of Multimodal Large Language Models

Multimodal Large Language Models (MLLMs) are gaining increasing popularity in both academia and industry due to their remarkable performance in various applications such as visual question answering, visual perception, understanding, and reasoning. Over the past few years, significant efforts have been made to examine MLLMs from multiple perspectives. This paper presents a comprehensive review of 200 benchmarks and evaluations for MLLMs, focusing on (1)perception and understanding, (2)cognition and reasoning, (3)specific domains, (4)key capabilities, and (5)other modalities. Finally, we discuss the limitations of the current evaluation methods for MLLMs and explore promising future directions. Our key argument is that evaluation should be regarded as a crucial discipline to support the development of MLLMs better. For more details, please visit our GitHub repository: https://github.com/swordlidev/Evaluation-Multimodal-LLMs-Survey.

==> Draft/Implication_Understanding.tex <==
%TransportationGame:https://arxiv.org/abs/2401.04471
%MMVP:https://arxiv.org/abs/2401.06209
%MM-SAP:https://arxiv.org/abs/2401.07529
%AesBench:https://arxiv.org/abs/2401.08276
%Mementos:https://arxiv.org/abs/2401.10529
%CMMMU:https://arxiv.org/abs/2401.11944
% RTVLM:https://arxiv.org/abs/2401.12915
%CMMU:https://arxiv.org/pdf/2401.14011
%LHRS-Bench:https://arxiv.org/abs/2402.02544
%MULTI:https://arxiv.org/abs/2402.03173
% MHaluBench:https://arxiv.org/abs/2402.03190
% CorrelationQA:https://arxiv.org/abs/2402.03757
%SceMQA:https://arxiv.org/pdf/2402.05138
%Q-Bench+:https://arxiv.org/abs/2402.07116
%VQAv2-IDK:https://arxiv.org/abs/2402.09717
%Asclepius:https://arxiv.org/abs/2402.11217
%ChartX:https://arxiv.org/abs/2402.12185
%MAD-Bench:https://arxiv.org/abs/2402.13220
%CODIS:https://arxiv.org/pdf/2402.13607
%MM-Soc:https://arxiv.org/abs/2402.14154
%Math-Vision:https://arxiv.org/abs/2402.14804
%MMEcaption:https://arxiv.org/abs/2402.14973
% OSCaR:https://arxiv.org/abs/2402.17128
%CRPE https://arxiv.org/abs/2402.19474
% TempCompass:https://arxiv.org/abs/2403.00476
%Henna:https://arxiv.org/abs/2403.01031
%NPHardEval4V:https://arxiv.org/abs/2403.01777
%VLKEB:https://arxiv.org/abs/2403.07350
%MathVerse:https://arxiv.org/abs/2403.14624
%MDVP-Bench:https://arxiv.org/abs/2403.20271
%MMStar:https://arxiv.org/pdf/2403.20330
%M3D:https://arxiv.org/abs/2404.00578
%JailBreakV-28K:https://arxiv.org/abs/2404.03027
%FABABench:https://arxiv.org/abs/2404.05052
%Freet-UI:https://arxiv.org/abs/2404.05719
%VisualWebBench:https://arxiv.org/abs/2404.05955
%UNIAA:https://arxiv.org/abs/2404.09619
%CFMM:https://arxiv.org/pdf/2404.12966
%MARVEL:https://arxiv.org/abs/2404.13591
%DesignProbe:https://arxiv.org/abs/2404.14801
%ImplicitVAE:https://arxiv.org/abs/2404.15592
%MMT-Bench:https://arxiv.org/abs/2404.16006
%SEED-Bench-2-Plus:https://arxiv.org/abs/2404.16790
%Milebench:https://arxiv.org/abs/2404.18532
%Mile-Bench:https://arxiv.org/abs/2404.18532
%TableVQA-Bench:https://arxiv.org/abs/2404.19205
%Plot2Code:https://arxiv.org/abs/2405.07990
%SOK-Bench:https://arxiv.org/pdf/2405.09713
%MRHal-Bench:https://arxiv.org/abs/2405.11165
%MTVQA:https://arxiv.org/abs/2405.11985
%Video-MME:https://arxiv.org/abs/2405.21075
% SpatialRGPT:https://arxiv.org/abs/2406.01584
%MLVU:https://arxiv.org/abs/2406.04264
%M3GIA:https://arxiv.org/abs/2406.05343
%II-Bench:https://arxiv.org/abs/2406.05862
%-CVQA:https://arxiv.org/abs/2406.05967
% MultiTrust:https://arxiv.org/abs/2406.07057
%MM-NIAH:https://arxiv.org/abs/2406.07230
%MMWorld:https://arxiv.org/abs/2406.08407
%MMRel https://arxiv.org/abs/2406.09121
% ADLMCQ:https://arxiv.org/abs/2406.09390
%MuirBench:https://arxiv.org/abs/2406.09411
%Cog-Bench:https://arxiv.org/abs/2406.10424
%MMR:https://arxiv.org/abs/2406.10638
%MMNeedle:https://arxiv.org/abs/2406.11230
%-MC-MKE:https://arxiv.org/abs/2406.13219
%GSR-BENCH https://arxiv.org/abs/2406.13246
%Event-Bench:https://arxiv.org/abs/2406.14129
%VideoHallucer:https://arxiv.org/abs/2406.16338
%CV-Bench:https://arxiv.org/abs/2406.16860
%MM-SpuBench:https://arxiv.org/abs/2406.17126
%Charxiv:https://arxiv.org/abs/2406.18521
%MMRO:https://arxiv.org/abs/2406.19693
%Web2Code:https://arxiv.org/abs/2406.20098
% MIA-Bench:https://arxiv.org/abs/2407.01509
%CRAB:https://arxiv.org/abs/2407.01511
% ScanReason:https://arxiv.org/abs/2407.01525
%MathCheck:https://arxiv.org/abs/2407.08733
%-CHOPINLLM:https://arxiv.org/abs/2407.14506
%CompBench:https://arxiv.org/abs/2407.16837
%-MuChoMusic:https://arxiv.org/abs/2408.01337
%MMIU:https://arxiv.org/abs/2408.02718
%GMAI-MMBench https://arxiv.org/abs/2408.03361
%VisualAgentBench:https://arxiv.org/abs/2408.06327

==> Draft/draft.tex <==
############MDVP-Bench##############
To advance visual prompting research for MLLMs, we introduce MDVPData and MDVP-Bench.  MDVP-Bench, a comprehensive and challenging benchmark
to assess a model’s capability in understanding visual prompting instructions.
However, current MLLMs tend to focus on
comprehending entire images by aligning them with textual information at the
image level.To evaluate the effectiveness and robustness of visual prompting models,we introduce MDVP-Bench, a benchmark tailored for assessing models’ pixellevel comprehension. MDVP-Bench encompasses a variety of tasks, including
point-level and region-level captioning, which test the models’ ability to describe specific visual elements; inter-relationship analysis, assessing the understanding of connections between entities; and complex reasoning, challenging
the models’ ability to infer and deduce from visual information.
We introduce MDVP-Bench, a challenging benchmark designed to evaluate tasks that require a combination of detailed description referrals, interrelationship analysis, and complex reasoning.
MDVP-Bench is a comprehensive and challenging benchmark encompassing a
wide array of tasks, including concise descriptions, elaborate narratives, analyses of interconnections among different regions, and complex reasoning.
Existing evaluations typically follow the approach of LLaVA [35], utilizing
GPT-4 for open-ended evaluation and employing textual descriptions to depict
image content. These textual descriptions, often based on image annotations,
can lead to scenarios where GPT-4 may not recognize objects or backgrounds
not annotated in the scene. Additionally, inherent domain gaps between textual
descriptions and images can lead to GPT-4 misunderstanding the image content.
To address these limitations, we employ GPT-4V for evaluation in MDVP-Bench.


MME: A Comprehensive Evaluation Benchmark for Multimodal Large Language Models
Multimodal Large Language Model (MLLM) relies on the powerful LLM to perform multimodal tasks, showing amazing emergent abilities in recent studies, such as writing poems based on an image. However, it is difficult for these case studies to fully reflect the performance of MLLM, lacking a comprehensive evaluation. In this paper, we fill in this blank, presenting the first comprehensive MLLM Evaluation benchmark MME. 
It measures both perception and cognition abilities on a total of 14 subtasks.
Although these models exhibit surprising conversational
capabilities when conducting everyday chats, we still know
little about how well they quantitatively perform in various
aspects. The existing three common quantitative evaluation
manners for MLLMs have their limitations that are difficult
to comprehensively evaluate performance. Specifically, the
first manner  evaluates on existing traditional
multimodal datasets, such as image caption and VQA. However, on the one hand, it may be hard to reflect the emergent abilities of MLLMs on these datasets.
On the other hand, since the training sets of large models are
no longer unified, it is difficult to guarantee that all MLLMs
have not used the testing set for training. The second manner [48] is to collect data for an open-ended evaluation, but
either the data is unavailable to public by now  or the
amount is small (only 50 images) [48]. The third manner
focuses on one aspect of MLLMs, such as object hallucination [25] or adversarial robustness [56], which is powerless
to comprehensive evaluation.
In light of these concerns, a new comprehensive evaluation benchmark is urgently needed to match the flourish
of MLLMs. We argue that a universal comprehensive evaluation benchmark
30 advanced MLLMs are evaluated on MME and the
experimental results show that there is still a large room to
improve.
The first problem is not following instructions.Although we have adopted a very concise instruction design, there are MLLMs that answer freely
rather than following instructions.We argue that a good MLLM (especially after instruction tuning) should be able to follow such a simple
instruction, which is also very common in everyday life.
The second problem is a lack of perception.
 We notice that the performance of perception is vulnerable to
the nuance of instructions, since the two instructions of the
same image differ in only one word, but lead to completely
different and even contradictory perception results.
The third problem is a lack of reasoning.These
phenomena indicate that the logic chain is broken during the
reasoning process of MLLMs. Adding CoT prompts, such
as “Let’s think step by step” [13], may yield better results.
We look forward to a further in-depth research.
The fourth problem is object hallucination following instructions, This suggests an urgent need to suppress
hallucinations, and the community should take into account
of the reliability of the generated answers.

POPE:Evaluating Object Hallucination in Large Vision-Language Models
Despite the promising progress on LVLMs, we find that they suffer from object hallucinations, i.e., they tend to generate objects inconsistent with the target images in the descriptions. To investigate it, this work presents the first systematic study on object hallucination of LVLMs.
We conduct the evaluation experiments on several representative LVLMs, and show that they mostly suffer from severe object hallucination issues. We further
discuss that the visual instructions may influence the hallucination, and find that: objects that frequently appear in the visual instructions or co-occur with the image objects are obviously prone to be hallucinated by LVLMs.
In this work, we conducted evaluation experiments on several LVLMs and examined how they suffer from the object hallucination issue. By investigating the reasons for object hallucination, we empirically revealed that the object distributions of the visual instructions would affect the object hallucination of LVLMs. Besides, we also found that the existing hallucination evaluation methods might be affected by the input instructions and the generated text of LVLMs, thus leading to less reliable evaluation results. To address this issue, we proposed a polling-based query method called POPE, to provide an improved evaluation approach for the object hallucination of LVLMs. Experimental results have shown that our proposed POPE can better evaluate the object hallucination issue of LVLMs.
Limitations:First, we only focus on the object hallucination problem in
LVLMs, while do not consider other aspects that can reflect the capacities of LVLMs.

MMBench: Is Your Multi-modal Model an All-around Player?
However,
effectively evaluating these large VLMs remains a major challenge, hindering
future development in this domain. Traditional benchmarks like VQAv2 or COCO
Caption provide quantitative performance measurements but lack fine-grained ability assessment and robust evaluation metrics. Meanwhile, subjective benchmarks,
such as OwlEval, offer comprehensive evaluations of a model’s abilities by incorporating human labor, which is not scalable and may display significant bias. In
response to these challenges, we propose MMBench, a bilingual benchmark for
assessing the multi-modal capabilities of VLMs.
Given the aforementioned challenges, recent studies, such as OwlEval [49] and LVLM-eHub [48] propose human-involved subjective evaluation strategies, aiming to address existing methods’ limitations by incorporating human judgment and perception in the evaluation process. OwlEval artificially constructs 82 open-ended questions based on images from public datasets and employs human annotators to assess the quality of VLM predictions.These include accurate matching, where humans can precisely correlate a prediction with the target, even when expressed in different words, and comprehensive assessment, where humans are inclined to juxtapose two predictions considering multiple facets. The
ultimate score is computed as the mean score across diverse abilities, facilitating a holistic evaluation of the model’s capabilities.
MMBench is a systematically designed objective benchmark for a robust and holistic evaluation of vision-language models.
In light of the challenges faced by conventional objective and subjective benchmarks, we propose MMBench, a systematically designed objective evaluation benchmark to robustly evaluate different abilities of large vision-language models.
MMBench contains over 3000 multiple-choice questions covering 20 different ability dimensions, such as object localization and social reasoning,
for evaluating vision-language models. Each ability dimension encompasses over 125 questions, with the quantity of questions per ability maintained at a roughly equal level.
In order to reduce the number of false-negative samples during answer matching, we employ GPT-4 to match a model’s prediction to candidates choices in a multi-choice question and then output the label for the matched choice
We introduce MMBench, a multi-modality benchmark that performs objective evaluation for VLMs with over 3,000 multiple-choice questions covering 20 ability dimensions. To produce robust and reliable evaluation results, we introduce a new evaluation strategy named CircularEval. The strategy
is much stricter than the vanilla 1-pass evaluation and can yield reliable evaluation results at an affordable cost. Considering the limited instruction following ability of some VLMs, to yield more accurate evaluation results, we additionally adopt LLMs to extract choices from the model’s redictions. We comprehensively evaluate over 20 mainstream VLMs on MMBench, covering
different architectures and parameter sizes. The evaluation results provide valuable insights for future improvements.
Perception refers to gathering information from sensory inputs, while reasoning involves drawing conclusions based on this information.

MM-Vet: Evaluating Large Multimodal Models for Integrated Capabilities
Rapid model advancements pose challenges to evaluation benchmark development.
Problems include: (1) How to systematically structure and evaluate the complicated multimodal tasks; (2) How to design evaluation metrics that work well across question and answer types; and (3) How to give model insights beyond a simple performance ranking. To this end, we present MM-Vet, designed based on the
insight that the intriguing ability to solve complicated tasks is often achieved by a generalist model being able to integrate different core vision-language (VL) capabilities.
Despite the promising qualitative results on LMM’s capabilities, it remains unclear how to systematically evaluate those showcased complicated multimodal tasks and what are the relationships among evaluated tasks, which is the first step in developing a quantitative evaluation benchmark.
existing vision-language benchmarks [VQAv2, COCO, TextVQA] focus on simple Vision-Language (VL) tasks that require specific one or two capabilities, such as recognition, language generation, or OCR, but fall short in benchmarking more complicated tasks. Alternatively, we examine the arbitrary integration of core VL capabilities for complicated tasks,
MM-Vet defines six core VL capabilities, including recognition, OCR, knowledge,
language generation, spatial awareness, and math, which integrate to solve various complicated multimodal tasks.
We propose MM-Vet to evaluate LMMs’ ability on complicated multimodal tasks. MM-Vet defines 16 emergent tasks of interest, integrated from the six defined core VL capabilities.
Our MM-Vet is most related to the concurrent evaluation studies [27, 54, 45, 80, 50] such as MME and MMBench, which design comprehensive evaluation samples to facilitate the LMM evaluation.One major difference is that MM-Vet defines and studies the integrated VL capabilities, allowing the evaluation to provide insights beyond the overall model ranking.

LLaVA-Bench:Visual Instruction Tuning
We present the
first attempt to use language-only GPT-4 to generate multimodal language-image
instruction-following data.
To facilitate future research on visual
instruction following, we construct two evaluation benchmarks with diverse and
challenging application-oriented tasks.
Multimodal instruction-following benchmark. We present LLaVA-Bench with two challenging benchmarks, with a diverse selection of paired images, instructions and detailed annotations.
This benchmark studies the model’s alignment behavior and capabilities with consistent visual inputs. We vary the training datasets to study the effectiveness of different types of instruction-following data,
To evaluate the model’s capability in more challenging tasks and
generalizability to novel domains, we collect a diverse set of 24 images with 60 questions in total, including indoor and outdoor scenes, memes, paintings, sketches, etc., and associate each image with a highly-detailed and manually-curated description and a proper selection of questions.
This LLaVA-Bench (In-the-Wild) is designed to be challenging and to reveal a model’s weaknesses. We provide two examples with associated captions and questions in Table 6. For the ramen example (left), to correctly answer the name of the restaurant, it requires the model to have a large knowledge coverage and multilingual understanding capability; to correctly describe the
side dishes, the model may need to retrieve relevant multimodal information from Internet. For the fridge example (right), perceiving the correct brand of the yogurt requires the model to process high
resolution images and possess extensive knowledge coverage. 
we present the first benchmark to study multimodal instruction following capability. 

TouchStone: Evaluating Vision-Language Models by Language Models
Recently, MME (Fu et al., 2023) has been proposed to transform questions into
binary judgment statements for large model evaluation. MMBench (Liu et al., 2023b) evaluates models based on their accuracy in choosing answers. However, the binary judgment and the ability to choose an answer may not fully capture the complexity in open-ended real-world dialogues, thereby limiting their suitability as a comprehensive evaluation method.To tackle these challenges, we propose an automated evaluation method termed TouchStone, which provides
a comprehensive assessment of the capabilities of multimodal language models. The principles of our design are two-fold:
Firstly, in order to evaluate the overall abilities of the models, we construct a comprehensive visual dialogue dataset, encompassing five major categories of abilities and 27 subtasks. These categories include basic descriptive ability, visual recognition ability, visual comprehension ability, visual storytelling ability, and multi-image analysis ability. This not only tests the model’s recognition and comprehension abilities but also tests its literary creation and analysis abilities. 
Secondly, TouchStone involves converting information from other modalities, such as images, into textual forms by utilizing detailed image annotations and descriptions. This enables the employment of advanced LLMs to directly assess the quality of dialogues without the requirements for human evaluators or visual augmented LLMs. 
Addressing these limitations, our research aims to develop a novel evaluation methodology that directly compares the conversation to assess the performance of vision-language models. Concurrent with our work, VisIT-Bench (Bitton et al., 2023) also incorporates human annotations and advanced LLMs as evaluators. However, they specifically focus on instruction-following capability by utilizing instruction-conditioned captions. In contrast, our approach involves a comprehensive assessment that encompasses various aspects of model performance while also considering model hallucinations
We curate a diverse visual dialogue dataset that covers five categories of abilities and 27 subtasks, encompassing not only basic recognition and comprehension but also extending to literary creation.
• TouchStone converts information from other modalities, such as images, into textual forms using detailed
annotations. This allows advanced language models to directly assess dialogue quality without manual
intervention. We show that GPT-4 can serve as a reasonable evaluator to evaluate the quality of LVLMs’ response. Specifically, in our experiment, we find that GPT-4 shows highly-consistent judgment compared to
human preference.

OwlEval:mPLUG-Owl : Modularization Empowers Large Language Models with Multimodality
We carefully build a visually-related instruction evaluation set OwlEval.
We carefully construct an instruction evaluation set, dubbed OwlEval, to assess the capabilities of different models in the context of visual-related tasks.
In order to comprehensively evaluate various models, we construct a visually-related evaluation set OwlEval by collecting 82 artificially constructed questions based on 50 images,
Partial images have multiple rounds of questions, refers to multi-turn conversation cases. These questions examine a variety of model capabilities including natural image understanding, diagram and flowchart
comprehension, optical character recognition (OCR), multi-modal creation, knowledge-intensive QA, and referential interaction QA.
As questions are open-ended, we employ manual evaluation
metrics to rate the model’s responses as A, B, C, or D following the rating method proposed in Self-Instruct

GVT-Bench:
To effectively evaluate MLLM’s visual understanding capacity at different levels, we curate a new benchmark (GVTBench) which includes both semantic understanding tasks (VQA and image captioning) as well as fine-grained visual understanding tasks (Object Counting and Multi-Class Identification). Based on GVTBench, we perform extensive experiments to study what makes for a good visual tokenizer for MLLMs
In order to quantify MLLM’s visual understanding capability,
Existing vision-language tasks mainly focus on semantic
understanding, but fine-grained visual perception is 非常关键的 for exploring whether the visual tokenizer is optimal for MLLMs. In order to know  what makes for a good visual tokenizer, GVT-bench was designed to especially evaluate an MLLM’s fine-grained visual perception by Object Counting and multi-class Identification, but 其中的数据 are  constrained in relatively small resolutions .

MagnifierBench:
we introduce MagnifierBench, an evaluation framework designed to scrutinize models’ ability to discern minute details and spatial relationships of small objects.
including MagnifierBench: a novel
benchmark we developed that focuses on evaluating LMMs’ capacity to detect minute details in highresolution images. The images in MagnifierBench showcase intricate scenes densely populated with
small objects, primarily found in first-person videos of household activities.
We introduce MagnifierBench, a unique benchmark focused on assessing the capabilities of
modern LMMs in recognizing minute attributes and inter-object relationships within large
images.*** introduce the MagnifierBench, extend the input resolution to a much larger range to fill this gap, which can test the ability to discern the details of small objects in high-resolution input
images

To assess the MLLMs’s understanding of nuanced visual-linguistic concepts, several benchmarks have been proposed. Winoground was created with a focus on compositional understanding. VALSE and VLChecklist investigate several linguistic phenomena by transforming real captions into confusing alternatives.   ARO [39] diagnoses VLMs in attribution, relation and ordering. Eqben [32] assesses whether the model is sensitive to visual semantic changes. Most existing benchmarks solely focus on subtle textual changes [12, 19, 21, 39, 42], as crafting confusing text candidates is straightforward that can be achieved through either LLMs or simple rules. Winoground [39] and Eqben [32] are most relevant to us, since we focus on minimal semantic changes in both images and texts, enabling a more comprehensive evaluation across modalities. However, the scale of Winoground is restricted by its costly curation, and the image diversity of Eqben is limited by virtual engines. In contrast, our data construction pipeline is scalable and can produce diverse images.

COMPBench\cite{kil2024CompBench} assessed the comparative understanding abilities of MLLMs across various dimensions by comparing two related images. 

SCIENCEQA is collected from elementary and high school science curricula

==> Figure/fig-numpapers.tex <==
\begin{tikzpicture}
\pgfplotstableread{
Year Papers
2020 0
2021 3
2022 3
2023.01 2
2023.02 7
2023.03 12 
2023.04 15
2023.05 22
2023.06+ 33
}\datatable

\begin{axis}[
    % width=.48\textwidth,
    % xlabel={Years},
    ylabel={Number of papers},
    xtick={1,2,3,4,5,6,7,8,9},
    xticklabels={2020,2021,2022,2023.01,2023.02,2023.03,2023.04,2023.05,2023.06+},
    xticklabel style={rotate=45, anchor=north east},
    % xlabel style={yshift=-10pt},
    ymin=0,
    ymax=35,
    ytick distance=5,
    legend pos=north west,
    ymajorgrids=true,
    grid=both,
    grid style=dashed,
    clip mode=individual,
    font=\small,
]

\addplot[color=blue, mark=triangle, mark options={fill=blue}] table[x expr=\coordindex+1, y=Papers] {\datatable};

\legend{Number of papers}
\end{axis}
\end{tikzpicture}



==> Figure/fig-tree.tex <==
\begin{forest}
  for tree={
  grow=east,
  reversed=true,
  anchor=base west,
  parent anchor=east,
  child anchor=west,
  base=left,
  font=\huge,
  rectangle,
  draw,
  rounded corners,align=left,
  minimum width=2.5em,
  inner xsep=4pt,
  inner ysep=1pt,
  },
  where level=1{
    text width=10em,
    fill=blue!20,
    font=\huge % 1级字号
  }{},
  where level=2{
    text width=5em,
    font=\LARGE, % 2级字号
    fill=pink!30
  }{},
  where level=3{
    font=\large, % 3级字号
    yshift=0.26pt,
    fill=yellow!20
  }{}
  % where level=1{text width=5em,fill=blue!10}{},
  % where level=2{text width=5em,font=\footnotesize,fill=pink!30}{},
  % where level=3{font=\footnotesize,yshift=0.26pt,fill=yellow!20}{},
  [MLLMs \\ Evaluation,fill=green!40
    [Comprehensive \\ Evaluation, text width=15em
        [Image, text width=5em
            [
            MDVP-Bench\cite{lin2024MDVP-Bench};
            MMBench\cite{liu2024MMBench};
            LLaVA-Bench\cite{liu2023LLaVA-Bench};
            MME\cite{MME};
            MM-Vet\cite{yu2023MM-Vet}; TouchStone\cite{bai2023TouchStone};
            ChEF\cite{shi2023ChEF}; 
            OwlEval\cite{ye2024OwlEval}
            ]
        ]
        [Video, text width=5em
            [
            Perception Test\cite{pătrăucean2023PerceptionTest};
            MVBench\cite{li2024MVBench};
            Video-MME \cite{fu2024Video-MME};
            MMWorld\cite{he2024MMWorld};
            Video-Bench\cite{ning2023Video-Bench}
            ]
        ]
        [Omni-modal, text width=10em
            [
            SEED-Bench\cite{li2023SEED-Bench};
            SEED-Bench-2\cite{li2023SEED-Bench-2};
            Open-VQA\cite{zeng2023Open-VQA};
            MCUB\cite{chen2024MCUB}; 
            CRAB\cite{xu2024CRAB}
            ]
        ]
    ]
    [Visual \\ Perception, text width=10em
        [Fine-grained \\ Perception,text width=10em
            [\emph{Visual Grounding and Object Detection} \\
            Flickr30k Entities\cite{plummer2016Flickr30kEntities};
            Visual7W\cite{zhu2016Visual7W};
            V*Bench\cite{wu2023V*Bench};
            CODE\cite{zang2023CODE};
            ScanQA\cite{azuma2022ScanQA}
            ]
            [\emph{Counting and Fine-Grained recognition:} \\
            GVT-Bench\cite{wang2023GVT-Bench}/
            V* Bench\cite{wu2023V*Bench}/
            SPEC\cite{peng2024SPEC}/
            CV-Bench\cite{tong2024CV-Bench}\\
            MMVP\cite{tong2024MMVP}/
            P2GB\cite{chen2024P2GB}/
            Visual CoT\cite{shao2024VisualCoT}/
            MagnifierBench\cite{li2023MagnifierBench}
            ]
            [\emph{Visual-linguistic Concepts understanding:} \\
            VALSE\cite{VALSE}/
            VL-Checklist\cite{zhao2023VL-CheckList}/
            Winoground\cite{thrush2022Winoground}/
            ARO\cite{yuksekgonul2023ARO}/ 
            Eqben\cite{wang2023Eqben}/
            MMVP\cite{tong2024MMVP}
            ]
        ]
        [Corse-grained \\Perception, text width=12em
            [\emph{Image Quality Assessment:} \\
            Q-Bench\cite{wu2024Q-Bench}/
            Q-Bench+\cite{zhang2024Q-Bench+}
            ]
            [\emph{multi-image understanding:} \\
            MultipanelVQA\cite{fan2024MultipanelVQA}/ Mementos\cite{wang2024Mementos}/ 
            CompBench\cite{kil2024CompBench}
            ]
            [\emph{Implication Understanding:} \\
            II-Bench\cite{liu2024II-Bench}/
            ImplicitAVE\cite{zou2024ImplicitAVE}
            ]
            [\emph{Emotional Understanding:} \\
            FABA-Bench\cite{li2024FABA-Bench}/
            EmoBench\cite{yang2024EmoBench}
            ]
            [\emph{Aesthetics Perception:} \\
            AesBench\cite{huang2024AesBench}/
            UNIAA\cite{zhou2024UNIAA}
            DesignProbe\cite{doris2024DesignQA}
            ]
        ]
    ]
    [Cognition \\ and Reasoning, text width=12em
        [General Reasoning, text width=17em
            [\emph{Comprehensive Reasoning:} \\
            Visual Madlibs\cite{yu2015VisualMadlibs}/
            ScanReason\cite{zhu2024ScanReason}
            ]
            [\emph{Visual Relation:} \\
            Visual Genome\cite{krishna2016VisualGenome}/
            GQA\cite{hudson2019GQA}/
            VSR\cite{VSR}/
            What'sUp\cite{kamath2023what'sup}/
            GSR-BENCH\cite{rajabi2024GSR-BENCH}/
            CRPE\cite{wang2024CRPE}/
            MMRel\cite{nie2024MMRel}
            ]
            [\emph{Context-sensitive Reasoning:} \\
            CODIS\cite{luo2024CODIS}/
            CFMM\cite{li2024CFMM}/
            ]
            [\emph{In-Context Learning:} \\
            CoBSAT\cite{zeng2024CoBSAT}/
            VL-ICL Bench\cite{zong2024VL-ICLBench}
            ]
            [\emph{Vision-Indispensable Capabilities:} \\
            CLEVR\cite{johnson2016CLEVR}/
            VQAv2\cite{goyal2017VQAv2}/
            GVQA\cite{agrawal2018GVQA}/
            GQA\cite{hudson2019GQA}/
            MMStar\cite{chen2024MMStar}
            ]
        ]
        [Knowledge-based \\ Reasoning, text width=16em
            [\emph{Knowledge-based Visual Question Answering:} \\
            KB-VQA\cite{wang2015KBVQA}/
            FVQA\cite{wang2017FVQA}/
            OK-VQA\cite{marino2019OK-VQA}/
            A-OKVQA\cite{schwenk2022A-OKVQA}/
            SOK-Bench\cite{wang2024SOK-Bench}
            ]
            [\emph{Knowledge Editing:} \\
            MMEdit\cite{cheng2024MMEdit}/
            MIKE\cite{li2024MIKE}/
            VLKEB\cite{huang2024VLKEB}/
            MC-MKE\cite{MC-MKE}
            ]
        ]
        [Intelligence \\ and Science, text width=10em
            [\emph{Intelligent Question Answering:} \\
	      CFMM\cite{li2024CFMM}/
            MARVEL\cite{jiang2024MARVEL}/
            VCog-Bench\cite{cao2024VCog-Bench}/
            M3GIA\cite{song2024M3GIA}
            ]
            [\emph{Mathematical Question Answering:} \\
	      NPHardEval4V\cite{fan2024NPHardEval4V}/ 
            Geometry3K\cite{lu2021Geometry3K}/
            MathVista\cite{lu2024MathVista}/
            MathVerse\cite{MathVerse}/
            MATHCHECK\cite{zhou2024MATHCHECK}/
            Math-Vision\cite{wang2024Math-Vision}
            ]
            [\emph{Multidisciplinary Question Answering:} \\
            ScienceQA\cite{lu2022ScienceQA}/
            MMMU\cite{yue2024MMMU}/ 
            CMMU\cite{he2024CMMU}/
            SceMQA\cite{liang2024SceMQA}/
            M3Exam\cite{zhang2023M3Exam}/
            CMMMU\cite{zhang2024CMMMU}
            ]
        ]
    ]
    [Specific Domains, text width=15em
        [Text-Rich Visual\\ Capabilities, text width=17em
            [\emph{Text-oriented Question Answering:} \\
            TextVQA\cite{singh2019TextVQA}/
            TextCaps\cite{sidorov2020TextCaps}/
            OCR-VQA\cite{mishraICDAR19OCR-VQA}/ 
            OCRBench\cite{liu2024OCRBench}/
            P2GB\cite{chen2024P2GB}
            ]
            [\emph{Document-oriented Question Answering:} \\
            DocVQA\cite{mathew2021DocVQA}/
            InfographicVQA\cite{mathew2021infographicvqa}/
            DUDE\cite{vanlandeghem2023DUDE}/
            MM-NIAH\cite{wang2024MM-NIAH}
            ]
            [\emph{Chart-oriented Question Answering:} \\
            AI2D\cite{kembhavi2016AI2D}/
            ChartQA\cite{masry2022ChartQA}/
            SciGraphQA\cite{li2023SciGraphQA}/ 
            ChartBench\cite{xu2024ChartBench}\\
            MULTI\cite{zhu2024MULTI}/
            ChartX\cite{xia2024ChartX}/
            CharXiv\cite{wang2024CharXiv}/
            CHOPINLLM\cite{fan2024CHOPINLLM}/
            MMC-Benchmark\cite{liu2024MMC-Benchmark}
            ]
            [\emph{Html-oriented Question Answering:} \\
            VisualWebBench\cite{liu2024VisualWebBench}/ Plot2Code\cite{wu2024Plot2Code}/
            Web2Code\cite{yun2024Web2Code}
            ]
            [\emph{Comprehension Evaluation:} \\
            TableVQA-Bench\cite{kim2024TableVQA-Bench}/
            SEED-Bench-2-Plus\cite{li2024SEED-Bench-2-Plus}
            ]
        ]
        [Decision-making\\ Agent, text width=15em
            [\emph{Embodied Decision-making:} \\
            OpenEQA\cite{OpenEQA2023}/
            EgoPlan-Bench\cite{chen2024EgoPlan-Bench}/
            PCA-EVAL\cite{chen2023PCA-EVAL}/
            PCA-Bench\cite{chen2024PCA-Bench}/
            MMRo\cite{li2024MMRo}/
            MMT-Bench\cite{ying2024MMT-Bench}
            ]
            [\emph{Mobile Agency:} \\
            Mobile-Eval\cite{wang2024Mobile-Eval}/
            Freet-UI\cite{you2024Ferret-UI}
            ]
        ]
        [Particular \\Applications, text width=12em
            [Charting New Territories\cite{roberts2024ChartingNewTerritories}/
            LHRS-Bench\cite{muhtar2024LHRS-Bench}/
            TransportationGames\cite{zhang2024TransportationGames}/
            DesignQA\cite{doris2024DesignQA}/
            Asclepius\cite{wang2024Asclepius}\\
            M3D\cite{bai2024M3D}/
            VizWiz\cite{gurari2018VizWiz}/
            MM-Soc\cite{jin2024MM-Soc}/
            PCA-Bench\cite{chen2024PCA-Bench}/
            OpenLane\cite{chen2022OpenLane}
            ]
        ]
        [Diverse cultures\\ and languages, text width=15em
            [CMMU\cite{he2024CMMU}/ 
            Peacock\cite{alwajih2024Peacock} / 
            LaVy-Bench\cite{tran2024LaVy}/
            MTVQA\cite{tang2024MTVQA}/
            CVQA\cite{romero2024CVQA}]
        ]
    ]
    [Key Capabilities, text width=15em
        [Conversation Abilities, text width=17em
            [\emph{Long-context Capabilities:} \\
            Mile-Bench\cite{song2024MileBench}/
            MMNeedle\cite{wang2024MMNeedle}/
            MLVU\cite{zhou2024MLVU}/ 
            VNBench\cite{zhao2024VNBench}
            ]
            [\emph{ Instruction Following:} \\
            MIA-Bench\cite{qian2024MIA-Bench}/
	      DEMON\cite{wang2023DEMON}/
	      CoIN\cite{chen2024CoIN}/
	      VisIT-Bench\cite{bitton2023VisIT-Bench}/
	      LAMM\cite{florio2023LAMM}/
            ]
        ]
        [Hallucination, text width=12em
            [\emph{Causes and Classification:} \\
            POPE\cite{li2023POPE}/
            GAVIE\cite{liu2024GAVIE}/
            M-HalDetect\cite{wang2023M-HalDetect}/
            HaELM\cite{wang2023HaELM}\\
            Bingo\cite{cui2023Bingo}/ HallusionBench\cite{guan2024HallusionBench}/
	      CorrelationQA\cite{han2024CorrelationQA}/
            VHTest\cite{huang2024VHTest}
            ]
            [\emph{Quantification Methods:} \\
            MMHAL-BENCH\cite{sun2023MMHAL-BENCH}/
            CHAIR\cite{rohrbach2019CHAIR}/
            AMBER\cite{wang2024AMBER}/
	      MMECeption\cite{cao2024MMECeption}/
            MRHal-Bench\cite{sun2023MMHAL-BENCH}
            ]
            [\emph{Comprehensive Evaluation:} \\
            MHaluBench\cite{chen2024MHaluBench}/
	      VideoHallucer\cite{wang2024VideoHallucer}
            ]
        ]
        [Trustworthiness, text width=14em
            [\emph{Robustness:}\\
            MAD-Bench\cite{qian2024MAD-Bench}/
            MMR\cite{liu2024MMR}
	      MM-SpuBench\cite{ye2024MM-SpuBench}/
            MM-SAP\cite{wang2024MM-SAP}/
	      BenchLMM\cite{cai2023benchlmm}/
            VQAv2-IDK\cite{cha2024VQAv2-IDK}
            ]
            [\emph{Safety:}\\
            MMUBench\cite{li2024MMUBench}/
            SHIELD\cite{shi2024SHIELD}/
	      MM-SafetyBench\cite{liu2024MM-SafetyBench}/
            JailBreakV-28K\cite{luo2024JailBreakV-28K}\\
	      Red Teaming GPT-4V\cite{chen2024RedTeamingGPT-4V}/
            VQAv2-IDK\cite{cha2024VQAv2-IDK}
            ]
            [\emph{Comprehensive Evaluation:}\\
            MultiTrust\cite{zhang2024MultiTrust}/
	      RTVLM\cite{li2024RTVLM}
            ]
        ]
    ]
    [Other Modalities, text width=12em
        [Videos, text width=7em
            [\emph{Temporal and Event Understanding:}\\
            MLVU\cite{zhou2024MLVU}
            VNBench\cite{zhao2024VNBench}/
            Event-Bench \cite{du2024Event-Bench}/
            MovieQA\cite{tapaswi2016MovieQA}/
            TempCompass\cite{liu2024TempCompass}/
            TimeIT\cite{Ren2023TimeIT}
            ]
            [\emph{State transition understanding and prediction:}\\
            OSCaR\cite{nguyen2024OSCaR}/
            WorldNet-Crafted\cite{ge2024WorldNet-Crafted}
            ]
        ]
        [3D Scenes, text width=10em
            [SQA3D\cite{ma2023SQA3D}/
            LAMM\cite{lamm}/
            GPT4Point\cite{qi2023GPT4Point}
            ]
        ]
        ]
    ]
  ]
\end{forest}
